VertiBench: Advancing Feature Distribution Diversity in Vertical Federated Learning Benchmarks

Vertical Federated Learning (VFL) is a crucial paradigm for training machine learning models on feature-partitioned, distributed data. However, due to privacy restrictions, few public real-world VFL datasets exist for algorithm evaluation, and these represent a limited array of feature distributions. Existing benchmarks often resort to synthetic datasets, derived from arbitrary feature splits from a global set, which only capture a subset of feature distributions, leading to inadequate algorithm performance assessment. This paper addresses these shortcomings by introducing two key factors affecting VFL performance - feature importance and feature correlation - and proposing associated evaluation metrics and dataset splitting methods. Additionally, we introduce a real VFL dataset to address the deficit in image-image VFL scenarios. Our comprehensive evaluation of cutting-edge VFL algorithms provides valuable insights for future research in the field.

==> section/junyiplot.tex <==
\subsection{Visualization of CIFAR10 and MNIST}\label{sec:exp-comm}

\todo{Add some descriptions about post-process of split}
% 给 CIFAR10 切分的空地涂成 255 （白色）%
% 给 MNIST 切分的地方涂成 0 （黑色），因为 MNIST 的背景是黑色的 %






==> section/real-datasets.tex <==
% \wzm{Although synthetic datasets can effectively simulate a wide range of VFL scenarios, obtaining a sufficient number of real datasets that encompass different scenarios remains the ideal approach.} Real-world VFL datasets currently encompass various data types, including tabular-tabular (as in Vehicle~\cite{duarte2004vehicle}, Movielens~\cite{hu2022oarf}, and Songs~\cite{hu2022oarf}) and tabular-image (as in NUS-WIDE~\cite{nuswide}). However, these benchmarks lack image-image datasets. To fill this gap, we present a real-world VFL dataset, \textit{Satellite}, which contains 62,832 images distributed over 16 parties. This dataset simulates a practical VFL scenario where multiple parties, each owning unique satellites, collaborate on a location identification task. These images captured by different satellites are linked on location IDs, enabling the classification of land types of these locations. Although Satellite comprises data from 16 visits by satellites owned by a single organization, it adequately simulates a realistic VFL scenario wherein multiple parties possess different satellites. A detailed description of the construction of the Satellite dataset is presented in Appendix~\ref{sec:satellite}.

% To conduct an in-depth analysis of the Satellite dataset distribution, we employ our proposed metrics, evaluate, and visually present the absolute values of correlation within this dataset, as illustrated in Figure~\ref{fig:corr-satellite}. For comparative purposes, we similarly evaluate the correlation within the NUS-WIDE dataset, as seen in Figure~\ref{fig:corr-wide}. Our observations reveal that both datasets exhibit low inter-party correlation (Icor) and high inner-party correlation, aligning with scenarios associated with small values of $\beta$. This further underscores that random feature splits, which typically result in larger $\beta$ values (as shown in Figure~\ref{fig:pcor-shuffle}), may not accurately mimic real-world cases. This observation is consistent with the position of shuffled real datasets in Figure~\ref{fig:real-dist}.


Real-world VFL datasets, though highly desirable, are limited in scope and type, often encompassing tabular-tabular data, as in Vehicle~\cite{duarte2004vehicle}, Movielens~\cite{hu2022oarf}, Songs~\cite{hu2022oarf}, and tabular-image data, as in NUS-WIDE~\cite{nuswide}. Notably missing are image-image datasets. Addressing this, we introduce a real-world VFL dataset, \textit{Satellite}, adapted from~\cite{satellite}, containing 62,832 images across 16 parties, simulating a practical VFL scenario of collaborative location identification via multiple satellites. 


\reva{Derived from the WorldStrat dataset~\cite{satellite}, the Satellite dataset comprises Points of Interest (POI) associated with 3,927 distinct Areas of Interest (AOI). Each AOI is characterized by a unique identifier, a land type, and 16 images from separate satellite pass-overs, signifying 16 parties for each geographic region. Labels are directly taken from WorldStrat's folder names. During preprocessing, 67 incomplete records were omitted, and all images were resized to 158x158 pixels, with pixel intensities adjusted to $[0,255]$. These images are categorized into four land types: \texttt{Amnesty POI} (4.8\%), \texttt{ASMSpotter} (8.9\%), \texttt{Landcover} (61.3\%), and \texttt{UNHCR} (25.0\%). Comprehensive dataset specifics are available in Appendix~\ref{sec:satellite}.}

% \reva{
% The Satellite dataset, derived from the WorldStrat dataset~\cite{satellite}, comprises Points of Interest (POI) linked to an Area of Interest (AOI). Each AOI has a unique identifier, a land type, and 16 distinct satellite images, with each image originating from a separate satellite pass-over. Therefore, for all 3,927 AOIs, there are 16 distinct satellite visits, effectively resulting in 16 parties capturing images for every location. During the refinement process, 67 incomplete records were excised, and all images were standardized to 13-channel 158x158 pixels with pixel values scaled to the $[0,255]$ range. The primary task is to classify images into four land type categories: \texttt{Amnesty POI} (4.8\%), \texttt{ASMSpotter} (8.9\%), \texttt{Landcover} (61.3\%), and \texttt{UNHCR} (25.0\%). For channel specifics, refer to the appendix.
% }

% An in-depth analysis of the Satellite dataset, using our proposed metrics and the visualization of absolute correlation matrix (Figure~\ref{fig:corr-satellite}), reveals low inter-party correlation (Icor) and high inner-party correlation, similar to NUS-WIDE (Figure~\ref{fig:corr-wide}). These results underscore the fact that random feature splits, which usually result in larger $\beta$ values (Figures~\ref{fig:pcor-shuffle} and \ref{fig:real-dist}), may not truly represent real-world scenarios, reinforcing the need for systematic VFL datasets generation methods.



==> section/related-work.tex <==
% \textbf{Vertical federated learning datasets.}
% The scarcity and limited range of real-world VFL datasets~\cite{nuswide,hu2022oarf,duarte2004vehicle} in benchmarks and studies~\cite{he2020fedml,caldas2018leaf} underscore the need for synthetic VFL datasets capable of depicting a broader spectrum of scenarios. Given VFL's focus on data privacy, obtaining such real datasets is challenging. Synthetic benchmarks~\cite{he2020fedml,caldas2018leaf} and VFL study datasets~\cite{diao2022gal,vepakomma2018split,cheng2021secureboost} commonly rely on unexplained random or manual feature splitting, which often represents scenarios of balanced feature importance and high inter-party correlation (Figure~\ref{fig:corrsplit},~\ref{fig:real-dist}). This situation indicates a pressing demand for systematic methods to generate synthetic VFL datasets that accurately reflect a diverse set of scenarios, fostering comprehensive evaluation of VFL algorithms.   % Removed for redundancy


% Real-world VFL datasets have been infrequently incorporated into VFL benchmarks~\cite{he2020fedml,caldas2018leaf} and are seldom utilized in VFL studies, as evidenced in Table~\ref{tab:vfl-algorithms}. The limited number of existing real VFL datasets~\cite{nuswide,hu2022oarf,duarte2004vehicle} only cater to a narrow range of VFL scenarios, as observed in Figure~\ref{fig:real-dist}. The premise of VFL is the inherent privacy and sensitivity of local data, thereby intensifying the challenge of obtaining real VFL datasets. This emphasizes the significance of synthetic VFL datasets that can depict a broader range of scenarios. Unfortunately, the majority of synthetic benchmarks~\cite{he2020fedml,caldas2018leaf} and experimental datasets in VFL studies~\cite{diao2022gal,vepakomma2018split,cheng2021secureboost} resort to random or manual feature splitting, with little to no explanation or analysis of their representativeness. Such evenly random feature partitioning tends to cover only a narrow scope of scenarios where parties share balanced feature importance and high inter-party feature correlation, as empirically shown in Figure~\ref{fig:corrsplit} and Figure~\ref{fig:real-dist}. Therefore, a pressing need arises for systematic methods capable of generating representative synthetic VFL datasets for a comprehensive evaluation of VFL algorithms across a wider range of scenarios.

\textbf{Feature importance.} The Shapley value~\cite{cohen2005feature,kumar2020problems,ma2020predictive}, used to assess party contributions in federated learning~\cite{wang2019measure,wang2019interpret,han2021data}, has significant computational costs, rendering it unsuitable for guiding feature splitting. Certain methodologies~\cite{li2022federated,li2022fedtree} utilize a Dirichlet distribution for global dataset random split, creating imbalanced federated learning datasets. However, they do not consider the partitioning of features of varying importance.

\textbf{Feature correlation.} The task of efficiently gauging correlation among two groups of features is challenging despite well-studied individual feature correlation~\cite{myers2004spearman,de2016comparing}. The Shapley-Taylor index, proposed for evaluating correlation between feature sets~\cite{sundararajan2020shapley}, is computationally intensive (NP-hard), and unsuitable for high-dimensional datasets. The determinant of the correlation matrix~\cite{wang2014measures} efficiently estimates inter-party correlation but is over-sensitive to linearly correlated features, impeding its use in feature partitioning. A more refined metric - the multi-way correlation coefficient (mcor)~\cite{taylor2020multi}, addresses this, but like the determinant, it struggles with unequal feature numbers across parties, a typical VFL scenario, due to the assumption of a square correlation matrix.

% \textbf{Feature Importance.} The Shapley value, a concept from game theory, has found application in quantifying feature importance in several studies~\cite{cohen2005feature,kumar2020problems,ma2020predictive}. Additionally, it has been introduced into federated learning~\cite{wang2019measure,wang2019interpret,han2021data} as a tool to assess each party's contribution. Despite these approaches accurately appraising the contribution and accounting for correlations among features, they frequently incur greater computational cost than the Shapley value, which is known to be an NP-hard problem. This computational burden renders the adoption of Shapley-value-based strategies in the feature partitioning a significant challenge. Certain methodologies~\cite{li2022federated,li2022fedtree} employ a Dirichlet distribution for the random split of global datasets, thereby creating imbalanced federated learning datasets. However, none of these approaches examine the division of features with different importance.





